Vision-LLMs Can Fool Themselves with Self-Generated Typographic Attacks

Typographic attacks, adding misleading text to images, can deceive vision-language models (LVLMs). The susceptibility of recent large LVLMs like GPT4-V to such attacks is understudied, raising concerns about amplified misinformation in personal assistant applications. Previous attacks use simple strategies, such as random misleading words, which don't fully exploit LVLMs' language reasoning abilities. We introduce an experimental setup for testing typographic attacks on LVLMs and propose two novel self-generated attacks: (1) Class-based attacks, where the model identifies a similar class to deceive itself, and (2) Reasoned attacks, where an advanced LVLM suggests an attack combining a deceiving class and description. Our experiments show these attacks significantly reduce classification performance by up to 60\% and are effective across different models, including InstructBLIP and MiniGPT4. Code: https://github.com/mqraitem/Self-Gen-Typo-Attack

==> Tables/Table_2.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{l|l}
\hline  
\multicolumn{1}{c|}{} & Avg \\ \hline
No Text &  99.3 \\
Typographic Attack & 98.0  \\
D-Typographic Attack (ours) & 94.0  \\
Model Based Typographic Attack (ours) &  \textbf{72.6}\\ \hline
\end{tabular}
\caption{Comparison between the effect of typographic attacks from prior work \cite{radford2021learning,azuma2023defense} and our new Reasoned Typographic Attack as well as Model Based Attacks using our benchmark as outlined in Section \ref{sec:def} on GPTV. Refer to Section \ref{sec:exp} for further discussion.}
\label{tb:table_1_main_results}
\end{table}


==> Tables/Table_3.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|c|cc|cccccc}
\toprule
\multicolumn{1}{c|}{} & No Attack & \multicolumn{6}{c}{Reasoned Typographic Attacks} \\ \midrule
$\hat{y}$ & - & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{T} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{T} & B \\
$M(x, i_d)^{\prime}$ & - & \multicolumn{1}{c|}{T} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{T} & \multicolumn{1}{c|}{T} & B \\ \midrule
LLaVA 1.5 & 85.5 & \multicolumn{1}{c|}{40.3} & \multicolumn{1}{c|}{38.8} & \multicolumn{1}{c|}{\textbf{17.0}} & \multicolumn{1}{c|}{21.8} & \multicolumn{1}{c|}{28.6} & 27.0 \\
InstructBLIP & 95.0 & \multicolumn{1}{c|}{47.6} & \multicolumn{1}{c|}{53.7} & \multicolumn{1}{c|}{21.3} & \multicolumn{1}{c|}{\textbf{17.5}} & \multicolumn{1}{c|}{30.2} & 23.9 \\
MiniGPT4 & 76.2 & \multicolumn{1}{c|}{52.8} & \multicolumn{1}{c|}{46.4} & \multicolumn{1}{c|}{\textbf{44.8}} & \multicolumn{1}{c|}{56.6} & \multicolumn{1}{c|}{51.9} & 45.1 \\
\bottomrule
\end{tabular}
\caption{Ablations over the effect of pasting the wrong class $\hat{y}$ and the deceiving description $M(x, i_d)$ at either the top (T) or the bottom (B) of the image. Note that results are averaged  over all the datasets defined in Section \ref{tab:table_2}. Refer to Section \ref{sec:pos_ablations} for further discussion.}
\label{tab:table_2} 
\end{table*}
